PyGFI: Analyzing and Enhancing Robustness of Graph Neural Networks Against Hardware Errors

Graph neural networks (GNNs) have recently emerged as a promising learning paradigm in learning graph-structured data and have demonstrated wide success across various domains such as recommendation systems, social networks, and electronic design automation (EDA). Like other deep learning (DL) methods, GNNs are being deployed in sophisticated modern hardware systems, as well as dedicated accelerators. However, despite the popularity of GNNs and the recent efforts of bringing GNNs to hardware, the fault tolerance and resilience of GNNs have generally been overlooked. Inspired by the inherent algorithmic resilience of DL methods, this paper conducts, for the first time, a large-scale and empirical study of GNN resilience, aiming to understand the relationship between hardware faults and GNN accuracy. By developing a customized fault injection tool on top of PyTorch, we perform extensive fault injection experiments on various GNN models and application datasets. We observe that the error resilience of GNN models varies by orders of magnitude with respect to different models and application datasets. Further, we explore a low-cost error mitigation mechanism for GNN to enhance its resilience. This GNN resilience study aims to open up new directions and opportunities for future GNN accelerator design and architectural optimization.

==> trash.tex <==
However, approximate computing based approaches will sacrifice accuracy in variant AI tasks. Another common technique for detecting and correcting errors is the use of error-correcting code (ECC), which involves adding redundant bits to data to enable the detection and correction of single-bit errors. While these techniques can help prevent SDC, they can also incur overhead in terms of cost, power consumption, and performance. For example, ECC typically requires additional memory or processing resources to perform error detection and correction, which can impact system performance and efficiency. Similarly, redundant components and diverse computing resources can increase system complexity and cost, as well as require additional power and cooling.

% having FI & testing built into widely used AI frameworks improves robustness/resiliency from SW to HW level

% Recently, designers are devising a scenario to continue the operations even in presence of errors, leading to \textit{approximate computing} which allows occasional errors in a system to appear as long as it delivers acceptable output quality. Specifically, recent research has shown that AI/ML models can exhibit a certain level of resilience or robustness to hardware errors, particularly in the presence of noisy or incomplete data~\cite{jiao2017assessment, zhang2018thundervolt}. For example, some studies have shown that certain types of neural networks, such as convolutional neural networks (CNNs) and recurrent neural networks (RNNs), can exhibit a degree of fault tolerance and resilience to hardware errors, which can help maintain performance in the presence of errors. Moreover, researchers have also explored the use of approximate computing techniques, which trade off accuracy for efficiency and can be particularly effective in the context of AI/ML, where small errors in computations may have minimal impact on the final output. These techniques can be leveraged to design more efficient hardware~\cite{reagen2016minerva, zhang2018thundervolt}, by reducing the precision or accuracy requirements of the computations and thereby reducing the energy consumption and hardware overhead.

Considering such a trade-off in both cases, it is significant to evaluate the error tolerance or error resilience of the conventional DL models. A feasible option for robustness evaluation is fault injection simulation. Recently, several studies present fault injection frameworks that target CNNs and RNNs error robustness ~\cite{reagen2018ares, mahmoud2020pytorchfi, kim2018matic}, which provides guidance to the deep learning model design from SW to HW level. As an important application in the DL field, GNNs are widely employed and deployed on non-Euclidean data. However, to the best of our knowledge, a comprehensive and systematic analysis of the GNNs fault injection framework has not been proposed yet.

% However, PyTorchFI cannot inject errors to GNNs because \textcolor{red}{XXX}. 

%When implementing PyGFI, we have also met some implementation challenges such as the quick consumption of the GPU memory due to the extremely large size of the GNN input and adjacency matrix. To alleviate this issue, we break the inference processing into batches to save the memory consumption. 

%introduce hook() 
% \begin{table}
% \centering
% \caption{}
%   \hspace{-20pt}
%     \begin{tabular}{cccc}
%     % \hline
%     \toprule
%     {Dataset}            & Cora    & Citeseer & Pubmed   & 
%     \hline
%     \\
%     \#Nodes & {2708}  & {3327}   & {19717} & 
%     \#Edges & {5429}  & {4732}   & {44338} & 
%     \#Features & {1433}  & {3703}   & {500}   & 
%     \#Categories & {7} & {6} & {3} & 
%     \bottomrule 
%     \end{tabular}
%   \label{tab:graph}
% \end{table}


% \begin{figure*}[t]
%     \centering



%     \label{fig:mitigation}
%     %\vspace{-15pt}
% \end{figure*}

% \begin{figure*}[t]
%     \centering

%     \subfigure[GCN]{
%         \includegraphics[width=0.8\columnwidth]{./figures/GCN_MITI.pdf}
%     }
%     \subfigure[GAT]{
%         \includegraphics[width=0.8\columnwidth]{./figures/GAT_MITI.pdf}
%     }
%     \subfigure[Chebyshev]{
%             \includegraphics[width=0.8\columnwidth]{./figures/CHEB_MITI.pdf}
%     }
%     \subfigure[SGC]{
%         \includegraphics[width=0.8\columnwidth]{./figures/SGC_MITI.pdf}
%     }
%     \vspace{-0.4cm}
%     \caption{GNNs accuracy after weight error mitigation (averaged over 3 datasets).}
%     \label{fig:mitigation}
%     \vspace{-0.5cm}
% \end{figure*}


% We explore Razor double-sampling based circuitry as a low-cost error masking technique to detect and mask errors~\cite{das2006self}, considering both NaN and non-NaN errors. Unlike parity bits protection~\cite{jahinuzzaman2009design} that can also detect memory fault but provides no information on the location of the affected bit, Razor-based method can detect erroneous bits and their locations. %In particular, upon the detection of bit flip(s), the faulty bit(s) will be set to 0. 
% The detailed implementations of Razor detection circuitry can be found in~\cite{das2006self, reagen2016minerva} and are out of the scope of this study. 

% We explore two error masking granularities at word-level and bit-level, respectively. For word masking, upon detecting any bit flips, it sets the entire word to 0. While for bit-level masking, it only recovers the faulty bit(s) to 0. Combined with Razor circuitry, both methods can be implemented with 0.3\% silicon area and 12.8\% power overheads on a single-port SRAM~\cite{reagen2016minerva}. As shown in Fig.~\ref{fig:mitigation}, we can see that bit-level masking always shows better robustness effects than word-level masking. Further, we notice that the word-level masking improves the inherent GNN robustness by up to $100X$ (cutoff rates from $10^{-6}$ to $10^{-4}$) while bit-level masking improves the robustness by up to $1000X$ (cutoff rates from $10^{-6}$ to $10^{-3}$). 

%This improved robustness can be translated to energy saving. For example, for a voltage-scaled on-chip SRAMs fabricated in FDX22 (22nm) technology~\cite{di2019pushing},  following the 
% That is being said, providing same performance, bit masking and word masking strategy can achieve 24.8\% and 13.2\% power saving respectively~\cite{zhang2022energy}. 
%In particular, upon the detection of bit flip(s), the faulty bit(s) will be set to 0.

% We explore Razor double-sampling-based circuitry as a low-cost error masking technique to detect and mask errors~\cite{das2006self}, considering both NaN and non-NaN errors. Unlike parity bits protection~\cite{jahinuzzaman2009design} that can also detect memory fault but provides no information on the location of the affected bit, Razor-based method can detect erroneous bits and their locations. %In particular, upon the detection of bit flip(s), the faulty bit(s) will be set to 0. 
% The detailed implementations of Razor detection circuitry can be found in~\cite{das2006self, reagen2016minerva} and are out of the scope of this study. 

% We explore two error masking granularities at word-level and bit-level, respectively. For word masking, upon detecting any bit flips, it sets the entire word to 0. While for bit-level masking, it only recovers the faulty bit(s) to 0. Combined with Razor circuitry, both methods can be implemented with 0.3\% silicon area and 12.8\% power overheads on a single-port SRAM~\cite{reagen2016minerva}. As shown in Fig.~\ref{fig:mitigation}, we can see that bit-level masking always shows better robustness effects than word-level masking. Further, we notice that the word-level masking improves the inherent GNN robustness by up to $100X$ (cutoff rates from $10^{-6}$ to $10^{-4}$) while bit-level masking improves the robustness by up to $1000X$ (cutoff rates from $10^{-6}$ to $10^{-3}$). 

%This improved robustness can be translated to energy saving. For example, for a voltage-scaled on-chip SRAMs fabricated in FDX22 (22nm) technology~\cite{di2019pushing},  following the 
% That is being said, providing same performance, bit masking and word masking strategy can achieve 24.8\% and 13.2\% power saving respectively~\cite{zhang2022energy}. 

% Further, we notice that the word-level masking improves the inherent GNN robustness by up to $100X$ (cutoff rates from $10^{-6}$ to $10^{-4}$) while bit-level masking improves the robustness by up to $1000X$ (cutoff rates from $10^{-6}$ to $10^{-3}$). 

%For the software-dominated mitigation approaches, we first mitigate all the NaN values to ``0'' since the NaN value is not a valid operation number within the clipping and filtering computation. 
%Then we apply clipping and filtering strategies to mitigate the influence of bit-flip error and retain the classification accuracy.

%the masking-based approaches can continuously protect the bit error and increase the robustness by 100X times. The clipping methods can provide acceptable protection by increasing the classification accuracy by 20\% on average. It is noticeable that in this paper we only utilize $[-1, 1]$ for the weight clipping which may not be the optimal values according to different parameters distribution across different models. In the future, we are deploying the weight clipping approach with a more precise threshold for better error mitigation performance.

%As the previous section mentioned, the basic clipping approach is not optimal for the error mitigation of variant weight matrices and activation outputs in GNNs models. According to our observation and experiments, the clipping-based approach has limited error-mitigating effects on activation errors. To this end, w

We further utilize the software-based error mitigation approaches, weight clipping and activation filtering, to mitigate the bit-flip error at the application level. Since the bit-flip error will deviate the original value out of the normal distribution, we can set a threshold to filter out the outliers (including NAN values) and decrease the impact of bit-flip errors. 

 
